Adaptable TeaStore: A Choreographic Approach

The Adaptable TeaStore has recently been proposed as a reference model for adaptable microservice architectures. It includes different configurations, as well as scenarios requiring to transition between them. We describe an implementation of the Adaptable TeaStore based on AIOCJ, a choreographic language that allows one to program multiparty systems that can adapt at runtime to different conditions. Following the choreographic tradition, AIOCJ ensures by-construction correctness of communications (e.g., no deadlocks) before, during, and after adaptation. Adaptation is dynamic, and the adaptation scenarios need to be fully specified only at runtime. Using AIOCJ to model the Adaptable TeaStore, we showcase the strengths of the approach and its current limitations, providing suggestions for future directions for refining the paradigm (and the AIOCJ language, in particular), to better align it with real-world Cloud architectures.

==> eptcsdata.tex <==
\providecommand{\firstpage}{79}
\providecommand{\publicationstatus}{G. De Palma and S. Giallorenzo (Eds.):\\
First Workshop on Adaptable Cloud Architectures\\
EPTCS 438, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.438.5}{10.4204/EPTCS.438.5}}
\pdfoutput=1
\usepackage{ifthen}
\providecommand{\eptcs}{{\sl Electronic Proceedings in Theoretical Computer Science}}
\providecommand{\opa}{, Open Publishing Association}
\providecommand{\finishreference}[6]{#1 #2#3, pp. #4--#5, \doi{10.4204/EPTCS.#2.#6}}
\providecommand{\thisvolume}[2][\eptcs]{%
 \ifthenelse{\equal{#2}{9}}{\finishreference{#1}{438}{\opa}{1}{14}{1}}{%
 \ifthenelse{\equal{#2}{4}}{\finishreference{#1}{438}{\opa}{40}{57}{3}}{%
 this volume of #1\opa}}}

